Constituent automorphism decoding of Reed-Muller codes

Automorphism-ensemble decoding is applied to the Plotkin constituents of Reed-Muller codes, resulting in a new soft-decision decoding algorithm with state-of-the-art performance versus complexity trade-offs.

==> table/SCL_comp.tex <==
\begin{tabular}{|c|c|c|}
\hline
Operations & list size & Corresponding equation \\ \hline
$2^{m-1}$ soft XOR & $\ell$ & (\ref{eq::GMC_LLRv})  \\ \hline
$2^{m-1}$ additions & $\ell'$ & (\ref{eq::GMC_LLRu})  \\ \hline
$2^{m-1}$ binary field addition & $\ell''$ & (\ref{eq::GMC concat})  \\ \hline
\end{tabular}

